Developmental Stage Classification of Embryos Using Two-Stream Neural Network with Linear-Chain Conditional Random Field

The developmental process of embryos follows a monotonic order. An embryo can progressively cleave from one cell to multiple cells and finally transform to morula and blastocyst. For time-lapse videos of embryos, most existing developmental stage classification methods conduct per-frame predictions using an image frame at each time step. However, classification using only images suffers from overlapping between cells and imbalance between stages. Temporal information can be valuable in addressing this problem by capturing movements between neighboring frames. In this work, we propose a two-stream model for developmental stage classification. Unlike previous methods, our two-stream model accepts both temporal and image information. We develop a linear-chain conditional random field (CRF) on top of neural network features extracted from the temporal and image streams to make use of both modalities. The linear-chain CRF formulation enables tractable training of global sequential models over multiple frames while also making it possible to inject monotonic development order constraints into the learning process explicitly. We demonstrate our algorithm on two time-lapse embryo video datasets: i) mouse and ii) human embryo datasets. Our method achieves 98.1 % and 80.6 % for mouse and human embryo stage classification, respectively. Our approach will enable more profound clinical and biological studies and suggests a new direction for developmental stage classification by utilizing temporal information.

==> sections/old/exp_another.tex <==
\subsection{Another Classification}

- Dataset (current datasets are not medical side, but can be seen as medical... in some sense)

Cardiology dataset

f-MRI

ECG/EKG dataset

\bfsection{Dataset}

\bfsection{Metric}

\bfsection{Result}


==> sections/old/methods_twostream.tex <==
\subsection{Dynamic Programming}

\bfsection{One Stream DP}

\bfsection{Two Stream DP}

==> sections/old/old_semisup.tex <==
\subsection{Semi-Supervised Learning of Two-Stream Model}
 
The main idea of FixMatch is to use augmented consistency and pseudo-label generation as a part of the training.

FixMatch tries to apply the model to two modified versions of the same image. It turns one of the predictions into a pseudo-label and tries to maximise the cross-entropy between the model prediction and the pseudo-label (unlabeled loss).

Then FixMatch uses the linear combination of a regular cross-entropy loss for the labeled data and unlabeled loss to train.

Our goal is to pre-train two independent models: model-rgb and model-flow. Model-rgb detects the stage of the embryo / it’s number of cells. Model-flow detects the change of the stage.

From here, our idea is to use one of these models as a replacement for the models in FixMatch with augmented inputs. I was not able to find a working way to turn model-flow outputs into the pseudo-labels for the model-rgb. But we are able to turn model-rgb outputs into the pseudo-labels as follows:

I consider the outputs of the model-rgb for the frames n and n-1. I calculate the softmaxed logits of the outputs of the proposed model for both frames. 

After that, I calculate the probability of change as   i!=endmodelrgb(n)stage i modelrgb(n-1)stage i-i  (where i is the index of the stage)


The probability of the end of the video as    modelrgb(end frame)  modelrgb(start frame)stage i-i 

And the probability of “no stage change” as 1 - rest. 

The argmax of these 3 is considered to be the pseudo-label for the model-flow.


==> tex-fig/dataset.tex <==
\begin{figure}[t]
     \centering
     %\includegraphics[width=\textwidth]{figures/dataset.pdf}
    %  \vspace{-0.2in}
     \caption{Samples in JWR-Mito300 and JWR-Pyr30 datasets. (a) Unlike textbook illustrations, mitochondria can have complicated 3D shapes. (b) Pyramidal neurons exhibit great diversity in the spatial distribution of dendrites and their branching patterns.}
     \label{fig:dataset}
     
\end{figure}


==> tex-fig/decomp.tex <==
\begin{figure}[t]
     \centering
     %\includegraphics[width=1.0\textwidth]{./figures/exp_decomp.pdf}
     \caption{3D shape decomposition with topological nonmenclatures. For mitochondrion (top row) and a pyramidal neurons (bottom row), we show the learned part dictionary and (b) greedy decomposition result for an input example.}
     \label{fig:decomp}
\end{figure}

==> tex-fig/method_old.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[height=1.5in]{figures/methods_old.svg}
     \caption{{\bf Two-stream CNN+HMM Model.}}
     \label{fig:method}
\end{figure}

==> tex-fig/retrieval.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[width=1.0\textwidth]{./figures/retrieval.pdf}
     \caption{Given (a) input 3D meshes, we show top-2 retrieval results for (b) our topological nomenclature, (c) Heat Kernel Signature (HKS), (d) spectral embedding.}
     \label{fig:retrieval}
\end{figure}

==> tex-tab/tab_results_ablation.tex <==

\begin{table}[h!]
    \centering
    \caption{Ablation study on the human embryo dataset.}
    \begin{tabular}{l|c}
    \hline %\hline
    Setting & Accuracy (\%)\\
    \hline
    Baseline  & 76.7 \\
    Baseline + Unary Potential & 80.0 \\
    Baseline + Unary Potential + Pairwise Potential & 80.6\\
    \hline
    \end{tabular}
    %\vspace{-0.2cm}
\label{table:ablation}
\end{table}


% \begin{table}[h!]
%     \centering
%     \caption{Ablation Study.}
%     \begin{tabular}{|c|c|c|}
%     \hline %\hline
%     Semi-Supervised & Linear-Chain CRF & Accuracy \\
%     \hline
%     & & 38.5\\
%     $\times$ & & \\
%     & $\times$ & \\ 
%     $\times$ & $\times$ &\\
%     \hline
%     % AP75&xx& xx & ?\\ 
%     \end{tabular}
%     %\vspace{-0.2cm}
% \label{table:ablation}
% \end{table}


